Taxonomy-as-a-Service: How To Structure Your Related Work

Structuring related work is a daunting task encompassing literature review, classification, comparison (primarily in the form of concepts), and gap analysis. Building taxonomies is a compelling way to structure concepts in the literature yielding reusable and extensible models. However, constructing taxonomies as a product of literature reviews could become, to our experiences, immensely complex and error-prone. Including new literature or addressing errors may cause substantial changes (ripple effects) in taxonomies coping with which requires adequate tools. To this end, we propose a \emph{Taxonomy-as-a-Service (TaaS)} platform. TaaS combines the systematic paper review process with taxonomy development, visualization, and analysis capabilities. We evaluate the effectiveness and efficiency of our platform by employing it in the development of a real-world taxonomy. Our results indicate that our TaaS can be used to effectively craft and maintain UML-conforming taxonomies and thereby structure related work. The screencast of our tool demonstration is available at \url{https://goo.gl/GsTjsP}.

==> parts/discussion.tex <==
\section{Discussion}\label{sec:discussion}
\subsection{Completeness and conformity}
In our evaluations, we showed that TaaS tools provide a complete tool-chain for both crafting and analyzing taxonomies.
The generated views and correlations perfectly conform to those presented in the software integrity protection taxonomy paper.
Nevertheless, our TaaS is primarily tailored for UML-conforming  taxonomies. 
Hence, it falls short to address other types of relations.
\subsection{Cropcircles, the hierarchical view}
The hierarchy analyzer can be useful for the verification of data quality and consistency as well as for finding gaps in the  literature. 
Furthermore, taxonomies can be traversed fast and the users can zoom into the sets of concepts of interest. 
However, inter dimensional and association relations cannot be captured in this view but only parent-child relationships. 
%For optimal results, every concept except for very few root nodes should have a parent specified. 
Clearly, the hierarchy is irrelevant for  taxonomies that barely include parent-child relations.

\subsection{Literature importer}
The keyword matching technique can facilitate the import of new literature into an ongoing taxonomy.
%This only results in a decent outcome if the concept names are specific enough and do not consist of multiple words. 
Nevertheless, the accuracy of results heavily depends on the papers and concepts that are being examined. 
This tool shall be solely seen as a facilitator for reviewing and subsequently importing new papers into taxonomies.
It by no means replaces the role of researchers in reading and classifying acquired papers.
Merely, it can be seen as a preliminary classification whereby researchers find potential matches for different concepts.
%Nevertheless, for some specific keywords (e.g., an emerging technology such as Intel SGX) keyword matching could be very effective.
%Whenever a string comparison technique that uses approximate string matching is being used, 
%it is recommended to check for every concept which variations of its name have been counted, to avoid semantic errors.

%Higher minimal occurrence counts seem to lead to better results. 
%A possible explanation is that single mentioning of a concept inside a paper 
%do not necessarily imply that the concept is being covered by it (as in being discussed in detail). 
%Nevertheless, these conformity values depend highly on the completeness of the manually acquired data. 
%The suitability of the considered concept names and papers for text parsing techniques, 
%that apply string comparison algorithms, plays a big role as well.

%The paper import functionality should primarily be seen as a tool that assists the user including papers, 
%that possibly cover a given set of concepts. 
%Although, a high occurrence count is a good indicator of this,
% further investigation by the researchers is essential, to make sure that a mapping is correct before it is being saved to the database. 
% The main use case of this functionality is to  lter out papers, which do not have to be examined further. 
% As a result the number of papers that have to be searched manually can be reduced. 
% Optimally, the parsing is being done multiple times with di erent methods and minimal similarities, 
% that take the syntax of the concept names into account. 
% The shorter the words and the more similar they are compared to other ones out of the same domain, 
% the higher the restrictions on the minimal similarity values have to be, to ensure a decent outcome.

==> parts/walkthrough.tex <==
\section{Walk Through}
There are two options to use the tool: on-premise and online demo. 
To run the tool on premise, users need to follow the installation guide available on the tools Github page accessible at \url{https://github.com/mr-ma/paper-review-go}.
We tried to minimize the effort for compilation and subsequently execution of the tool by resorting to a fully dockerized approach. 
Please note that basic familiarity with Docker and Docker Compose tools are mandatory. 

The alternative is to try the tool online accessible at \url{https://www22.in.tum.de/tools/integrity-taxonomy}.
To visit an already-crafted taxonomy no credentials whatsoever are needed. 
Users can simply select a taxonomy from the top menu and use correlation analyzers (2D and 3D) or hierarchy analyzer instantly.
However, editing or crafting a taxonomy naturally requires users to login the system. 
To facilitate the evaluation of the reviewers, we provide a test user credentials that can be used for editing or crafting a taxonomy.\\
\texttt{email: test@test.com} \\
\texttt{pass: FM5CPDub2EWmYp4g}\\
%For security reasons, the test user's access is restricted to one taxonomy, namely \texttt{demo}. 
To start crafting/editing a taxonomy, first you need to select your active taxonomy.
To do so, after logging in from the top menu click on \texttt{Taxonomy} $\rightarrow$ \texttt{demo}.
Afterward, the \texttt{Taxonomy Builder} button in the top menu opens the editor.  

Right click and hold on the default dimension (the rectangular box) displays a menu with options for adding dimensions and major nodes in the taxonomy editor.
Click on the circle of each empty dimension opens it (zooms into the dimension of interest). 
Double click on any empty space in zooms out of a dimension and takes the user to the interdimensional view.
Within each dimension right click and hold opens a menu with 4 operations: create major node, create node, remove and rename node. 
Hovering over nodes shows a gray circle click-and-hold on which enables users to model relations (by connecting elements).
All newly created relations are without any specialization type. 
Right click and hold on connections (edges) shows options for annotation, specialization of the relation, and further editing options.  
All the elements can be positioned simply with drag and drop. 
However, positions will only be persisted if the user explicitly clicks on the tiny save button on the top left hand side of the editor. 

Mapping papers to taxonomy nodes requires holding right click on a node and selecting \texttt{mapped papers}. 
Then, users can select the papers of interest from the available papers in the taxonomy metadata. 

Adding papers to a taxonomy can be done via the 2D correlation view or using the paper review process (accessible via the button to the right of taxonomy builder).
The paper review approach is fully explained in our demonstration video. Therefore, we refer the interested viewers to the screencast.
For an optimal paper import, users should craft a preliminary draft of their taxonomies.
This enables the use of keyword matching in the paper import process. 
Furthermore, users can add synonyms to each node of their taxonomy in the 2D correlation view.
Utilizing synonyms for concepts can improve the effectiveness of paper assignments to different taxonomy concepts.
All is needed to be done is to right click on the concepts in the correlation view and select synonyms.  
To import papers (in the 2D correlation view) click on the paper import button on the top left hand side of the view.
From the menu different algorithms and parameters can be set for the import procedure. 
Once the desired settings are set, clicking on the import papers button enables users to upload papers in pdf format.
The tool after selection of papers, attempts to map them to the concepts according to the matches keywords.
Thereafter, the imported papers are available in the taxonomy builder to be moved around between concepts throughout the development and maintenance of the taxonomy.

